Fast Mixed-Precision Real Evaluation

Evaluating real numbers to high precision is important in computational science, numerical computing, and in hardware and software design. Efficient algorithms exist for computing arithmetic operations and common elementary functions, but composing these primitives into larger expressions remains a challenge. The typical expression-evaluation algorithm computes all primitives in the expression to a uniform precision, doubling that precision until a sufficiently-accurate result is achieved. This is wasteful: usually only a few operations really need to be performed at high precision, and the bulk of the expression could be computed at a much lower, faster precision. However, no rigorous algorithm currently exists to compute these non-uniform precision assignments, nor to leverage non-uniform precision to reduce the number of primitive computations needed to evaluate an expression. We propose a new algorithm for deriving such rigorous precision assignments and reducing the number of primitive computations needed. This algorithm can leverage results computed at lower precisions to analytically determine a precision for each primitive that will result in a sufficiently-accurate evaluation. It can also use information from constant subexpressions, movability flags, and repeat flags to skip the computation of certain primitives, further reducing the time to evaluate real expressions. Our implementation, Reval, achieves an average speed-up of 3.97x compared to the widely-used Sollya tool, with the speed-up increasing to 9.26x on the most difficult inputs. A detailed evaluation shows that this speed-up results from both assigning lower precisions to the majority of primitives and from computing fewer primitives overall.

==> proof.tex <==
This section rigorously derives
  the results of \Cref{sec:bounds}.
The derivations are technical,
  and some readers may choose to skip this section.
The overall point is that \toolname's precision assignments
  are sound, meaning that they over-estimate the necessary precision,
  and typically fairly tight.

\subsection{Mathematical Background}

Error Taylor series,
  implemented in tools like FPTaylor~\cite{fptaylor},
  Hugo~\cite{hugo}, and Satire~\cite{satire},
  bound the floating-point error
  of a sequence of floating-point operations
  $\hat{z}_i = \hat{f}_i(\hat{x}_i, \hat{y}_i)$
  computing expression $\hat{z}$.
As in \Cref{sec:bounds}, we rewrite
  $\hat{z}_i = f_i(\hat{x}_i, \hat{y}_i)(1 + \varepsilon_i)$
  for some $|\varepsilon_i| < 2^{-p}$,
  at which point $\hat{z}$ is a real-valued function
  $\hat{z}(\vec{\varepsilon})$ of many $\varepsilon_i$,
  whose exact real result $z$ is $\hat{z}(\vec{0})$.

Error Taylor series observing
  that the $\varepsilon$ values are small.
A Taylor expansion of $\hat{z}$ in $\vec{\varepsilon}$
  therefore yields 
\[
\hat{z}(\vec{\varepsilon}) = \hat{z}(\vec{0}) + \sum_{\varepsilon} \varepsilon \frac{\partial \hat{z}}{\partial \varepsilon}(\vec{0}) + o(\varepsilon^2).
\]
The first term is the real result;
  the second term is called the ``first-order error'';
  and the third term is called the ``higher-order error'';
  the notion of error here is absolute error.

In the typical application of error Taylor series,
  the first- and second-order errors are then computed
  by taking symbolic derivatives of $\hat{z}$
  and bounded over some input range,
  typically using
  a global non-linear optimizer for first-order error
  and interval arithmetic for second-order error,
  ultimately resulting in a numeric upper bound on absolute error.
The higher-order error term is
  particularly expensive to compute, since it involves
  quadratically-many second derivatives;
  some tools like Satire~\cite{satire} ignore it.

Condition numbers simplify the computation of first-order error;
  while we first learned of the connection in ATOMU~\cite{atomu},
  the basic insight is just reverse-mode automatic differentiation.
Suppose one wishes to bound relative error,
  not absolute error, using error Taylor series.
One then needs to compute the first-order error
  divided by $\hat{z}$,
  which involves computing
$(\partial \hat{z} / \partial \varepsilon_i)(\vec{0}) / \hat{z}(\vec{0})$.
Condition numbers rearrange this computation into
  a sum of products
\[
\sum_p \prod_{f_j \in p} \Gamma_{f_j},
\text{ where }
\Gamma_f = \frac{x f'(x)}{f(x)}
\]
where the sum ranges over all \emph{paths} $p$
  of operations $f_j$
  from the root of the expression tree to some intermediate node.
For example, in the overview example
  $(1 - \cos(x)) / \sin(x)$,
  the path from the root to $\cos(x)$
  involves a division and a subtraction,
  while the path from the root to $\sin(x)$,
  involves just a division.
The condition numbers $\Gamma_{f_j}$ of those operations
  are multiplied together per-path and summed across paths.
The benefit of computing relative error in this way
  is that each $\Gamma_{f_j}$ is local to some $f_j$,
  while derivatives $\partial \hat{z} / \partial \varepsilon_i$
  involve the whole expression $\hat{z}$ at once.
That can allow, as in ATOMU~\cite{atomu},
  blaming specific operations that for high error.

\subsection{Sound First-Order Error}

To derive \Cref{eq:bound}, we proceed
  analogously to error Taylor series.
Consider a fixed sequence
  $\hat{z}_i = \hat{f}_i(\hat{x}_i, \hat{y}_i)$,
  of floating-point operations $\hat{f}_i$
  on input and output floating-point registers.
Rewrite $\hat{f}_i(\hat{x}_i, \hat{y}_i)
  = f_i(\hat{x}_i, \hat{y}_i) (1 + \varepsilon_i)$,
  for some $|\varepsilon_i| \le 2^{-p_i}$,
  where $p_i$ is the precision used for this operation.
Substitute in $\hat{x}_i$ and $\hat{y}_i$,
  themselves computed in prior instructions,
  and call the result $\hat{z}_i(\vec{\varepsilon})$.

We now consider how $\hat{z}_i$ varies with $\vec{\varepsilon}$.
Apply the Lagrange remainder theorem at order 1:%
\footnote{There are many variations
  of the Lagrange remainder theorem;
  the statement below is one of them
  but can also be seen as
  a corollary of the mean value theorem.}
\[
  \hat{z}_i(\vec{\varepsilon}) - \hat{z}_i(\vec{0})
  =
  \sum_{j \le i} \varepsilon_j \frac{\partial \hat{z}_i}{\partial \varepsilon_j}(\vec{\varepsilon^*})
\]
  for some $0 \le \vec{\varepsilon^*} \le \vec{\varepsilon} \le 2^{-p_i}$
  (or the symmetrical bound for $\varepsilon_j < 0$).
In this bound,
  $\vec{\varepsilon}$ represents the rounding error
  of a faithfully-rounded execution,
  so $\vec{\varepsilon^*}$ represents the rounding error
  of some other, also faithfully-rounded execution.

We know the maximum size of $\vec{\varepsilon}$,
  but not its signs, so we use the triangle inequality:
\[
\left| \frac{\hat{z}_i(\vec{\varepsilon}) - \hat{z}_i(\vec{0})}{z_i} \right|
 \le
\max_{\vec{\varepsilon^*}}
\left|
\sum_{j \le i}
\varepsilon_j
\frac{1}{z_i}
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} (\vec{\varepsilon^*})
\right|
\le
\max_{\vec{\varepsilon^*}}
\sum_{j \le i}
\left|
\varepsilon_j
\frac{1}{z_i}
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} (\vec{\varepsilon^*})
\right|
\le
\max_{\vec{\varepsilon^*}}
\sum_{j \le i} 2^{-{p_j}}
\left|
\frac{1}{z_i}
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} (\vec{\varepsilon^*})
\right|
\]
Note that this formula
  must maximizes over all $\vec{\varepsilon^*}$,
  whereas the standard first-order error Taylor series
  just considers $\vec{\varepsilon^*} = \vec{0}$.
At the core, this difference comes from
  error Taylor series applying the Lagrange remainder theorem
  to the \emph{second}-order Taylor term,
  instead of the \emph{first}-order Taylor term as done here.
Considering $\vec{\varepsilon^*}$ is complex but allows us to avoid
  the higher-order error term from standard error Taylor series.

\subsection{Linear-Time Error Bounds}

Next, we consider how \Cref{eq:bound}
  can be computed in $O(i)$ time.
This trick is to rearrange the formula algebraically;
  the derivation is similar to condition numbers
  or reverse-mode automatic differentiation.

Consider
  the $\partial \hat{z}_i / \partial \varepsilon_j$ term
  and substitute in
  $\hat{z}_i = f_i(\hat{x}_i, \hat{y}_i) (1 + \varepsilon_i)$.
Then we have two cases:
  either $i = j$ or $i > j$.
If $i = j$,
  we have
\[
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} =
\frac{\partial \hat{z}_i}{\partial \varepsilon_i} =
f_i(\hat{x}_i, \hat{y}_i),
\]
  because the $\hat{x}_i$ and $\hat{y}_i$ terms
  are independent of $\varepsilon_i$.
On the other hand, if $i > j$,
  then $\varepsilon_i$ is independent of $\varepsilon_j$,
  so we have
\[
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} =
(1 + \varepsilon_i) \left(
(\partial_1 f_i)(\hat{x}_i, \hat{y}_i)
\frac{\partial \hat{x}_i}{\partial \varepsilon_j}
+
(\partial_2 f_i)(\hat{x}_i, \hat{y}_i)
\frac{\partial \hat{y}_i}{\partial \varepsilon_j}
\right),
\]
where $\partial_1 f$ and $\partial_2 f$ refer to
  the derivatives of $f$ in its first and second arguments.
Performing some rearrangements
  and noting that $|\varepsilon_i| < 2^{-p_i}$,
  we now have:
\begin{align*}
\overbrace{
\max_{\vec{\varepsilon^*}}
\sum_{j \le i} 2^{-p_j}
\left|
\frac{1}{z_i}
\frac{\partial \hat{z}_i}{\partial \varepsilon_j} (\vec{\varepsilon^*})
\right|
}^{\bound(\hat{z}_i)}
&\le
2^{-p_i}
\overbrace{
\max_{\vec{\varepsilon^*}}\left|
\frac{f_i(x^*_i, y^*_i)}{f_i(x_i, y_i)}
\right|
}^{\intro(\hat{z}_i)}
\\&+
(1 + 2^{-p_i})
\left(
\max_{\vec{\varepsilon^*}}
\left|
  \frac{x_i (\partial_1 f_i)(x^*_i, y^*_i)}{f_i(x_i, y_i)}
\right|
\right)
\left(
  \max_{\vec{\varepsilon^*}}
  \sum_{j < i} 2^{-p_j}
  \left|
    \frac1{x_i}
    \frac{\partial \hat{x_i}}{\partial \varepsilon_j}
    (\vec{\varepsilon^*})
  \right|
\right)
\\&+
(1 + 2^{-p_i})
\underbrace{
\left(
\max_{\vec{\varepsilon^*}}
\left|
  \frac{y_i (\partial_2 f_i)(x^*_i, y^*_i)}{f_i(x_i, y_i)}
\right|
\right)
}_{\ampl_k(\hat{z}_i)}
\underbrace{
\left(
  \max_{\vec{\varepsilon^*}}
  \sum_{j < i} 2^{-p_j}
  \left|
    \frac1{y_i}
    \frac{\partial \hat{y_i}}{\partial \varepsilon_j}
    (\vec{\varepsilon^*})
  \right|
\right)
}_{\bound(\hat{y}_i)}
\end{align*}
  where $x^*_i$ and $y^*_i$ are $\hat{x}_i$ and $\hat{y}_i$
  evaluated at $\vec{\varepsilon^*}$.
Rewriting this gargantuan formula
  using the helper functions defined by the braces,
  we get \Cref{eq:cnum}.

The intuition behind this formula
  is that every operation $\hat{z}_i$
  introduces some error, approximately $2^{-p_i}$,
  and also amplifies error
  in its inputs
  by factors of approximately $\ampl_k(\hat{z}_i)$.
The error bound for $\hat{z}_i$
  then sums these three factors.
Readers familiar with condition numbers
  will immediately see the similarity
  between \Cref{eq:cnum}
  and the condition number formula
  $e_z = \mu + \Gamma_x e_x + \Gamma_y e_y$~\cite{atomu}.
However, condition numbers bound only the first-order error
  so are unsound, while \Cref{eq:cnum} is sound,
  which is why there are small, but necessary,%
\footnote{In fact, the name \ampl is a pun
  on both ``amplification factor'' and ''ample'' as in sound.}
  differences
  like the $\intro(\hat{z}_i)$ factor multiplying $2^{-p_i}$,
  the slight difference in definition
  between $\ampl_k(\hat{z}_i)$ and $\Gamma_k$,
  and the extra $1 + 2^{-p_i}$ term.

\subsection{Precision Tuning}

Next, solve \Cref{eq:cnum} for the $p_j$ terms.
Formally, we seek $p_j$ such that
  $\bound(\hat{z}_i) \le 2^{-t}$
  for some target precision $t$.
To do so, split the allowed $2^{-t}$ error equally
  among the three terms on the right hand side of \Cref{eq:cnum}:
\begin{align*}
\bound(\hat{z}_i) \le 2^{-t} &\Leftarrow
2^{-p_i} \intro(\hat{z}_i) \le \frac13 2^{-t}
\\&\land
(1 + 2^{-p_i}) \ampl_1(\hat{z}_i) \bound(\hat{x}_i) \le \frac13 2^{-t}
\\&\land
(1 + 2^{-p_i}) \ampl_2(\hat{z}_i) \bound(\hat{y}_i) \le \frac13 2^{-t},
\end{align*}
  where the left arrow is a reversed logical implication.

Take the first conjunction,
  bounding the introduced error, first.
Rearranging a little and noting that $\log_2 3 \le 2$,
  we have $p_i \ge t + 2 + \lceil \log_2 \intro(\hat{z}_i) \rceil$.
Likewise consider, say, the first amplified error term.
It can be rearranged into
  $-\log_2 \bound(\hat{x}_i) \ge t + \log_2(3 + 3\cdot2^{-p_i})
  + \log_2 \ampl_1(\hat{z}_i)$.
As long as $p_i \ge 2$,
  the term $\log_2 (3 + 3\cdot2^{-p_i}) \le 2$
  so we must bound $\hat{x}_i$'s error
  to at most $t + 2 + \lceil\log_2 \ampl_1(\hat{z}_i) \rceil$ bits.
That yields \Cref{eq:constraints}.

\subsection{Simple amplification factors}

Amplification factors
  $\lceil \log_2 \ampl_k(\hat{z}_i) \rceil$
  can be computed using exponent tricks
  similar to those discussed in \Cref{sec:tuning}
  for $\lceil \log_2 \intro(\hat{z}_i) \rceil$.
However,
  there is an additional challenge,
  because the definition of $\ampl_k$
  refers to $(\partial_k f_i)(x_i^*, y_i^*)$.
Its value is not known,
  and the interval $(\partial_k f_i)(\bar{x}_i, \bar{y}_i)$
  that contains it
  has typically \emph{not} been computed.
Different operators $f$ require different techniques
  to overcome this challenge.

For addition and subtraction, there's no problem at all:
  $\log_2 \ampl_1(\hat{x} + \hat{y})$ 
  is just equal to $\log_2 | x / z |$,
  which is included in $\log_2 | \bar{x} / \bar{z} |$
  and thus bounded by $\maxlog \bar{x} - \minlog \bar{z}$.
Subtraction likewise presents no difficulty.

For multiplication, an extra \logspan factor appears:
  $\log_2 \ampl_1(\hat{x} \cdot \hat{y})$
  is equal to $\log_2 | x y^* / x y |$;
  the $x$ terms cancel leaving a bound of $\logspan \bar{y}$.

Similarly, the amplification factor for the power function
  in its first argument,
\[
\ampl_1(\pow(\hat{x}, \hat{y})) =
\left|
\frac{x y^* \pow(x^*, y^* - 1)}{\pow(x, y)} \right| =
\left|
\frac{x y^* \pow(x^*, y^*)}{x^* \pow(x, y)} \right| =
\left|
y^* \frac{x}{x^*} \frac{z^*}{z} \right|,
\]
  results in the bound
  $\maxlog \bar{y} + \logspan \bar{x} + \logspan \bar{z}$.

Division, square and cube roots, exponents, and logarithms
  allow a similar algebraic rearrangement,
  producing a formula that uses
  only integer operations on \maxlog and \minlog
  of $\bar{x}$, $\bar{y}$, and $\bar{z}$.
The resulting ``exponent tricks'' formulas
  are shown in \Cref{tab:exp-exact}.

\subsection{Approximations}

However, for some operators,
  an approximation has to be performed
  to bound $(\partial_k f)(x, y)$
  via some computation over $x$, $y$, or $z$.
These approximations allow us to construct
  exponent trick formulas for $\ampl_k(f)$,
  that is,
  formulas that bound $\lceil \log_2 \ampl_k(f) \rceil$
  using only integer operations
  on \maxlog and \minlog
  of $\bar{x}$, $\bar{y}$, and $\bar{z}$.
  
\Cref{tab:exp_tricks} shows 
  all of the approximations used 
  and the exponent trick formulas they result in;
  the rest of this section merely contains
  detailed derivations for each row of that table.

\paragraph{Power}
The $\ampl_2$ factor for the power function $x^y$
  has uses a $\log(x^*)$ term.
This means that we must bound $\log_2 |\log(x)|$
  in terms of $\log_2 |x|$.
To do so, we first rewrite
\[
\log_2 |\log(x)| = \log_2 \left|\frac{\log_2(x)}{\log_2(e)}\right| = \log_2 |\log_2(x)| - \log_2 \log_2 e
\le \log_2 |\log_2(x)| - \frac12.
\]
Set $s = \log_2(x)$; since
  $\log_2 |s| \le |s| - \frac12$,
  we have $\log_2 |s| - \frac12 \le |s| - 1$.
This ultimately means that
  $\log_2 |\log(x^*)|$ is bounded above by
  $|\log_2 |\bar{x}|| - 1$.
That is just
  $\max(|\maxlog(\bar{x})|, |\minlog(\bar{x})|) - 1$.

\paragraph{Sine and Cosine}
The amplification factor for $\sin(x)$ involves $\cos(x)$.
Because $|\cos(x)| \le 1$, we have $\log_2 |\cos(x^*)| \le 0$;
  this allows us to show that
\[
  \lceil \log_2 \ampl_1(\sin(\hat{x})) \rceil \le \maxlog \bar{x} - \minlog \bar{z}.
\]

Likewise, for cosine we must bound $\sin(x)$;
  one simple approximation is
  $|\sin(x)| \le \min(|x|, 1)$,
  meaning $\log_2 |\sin(x^*)| \le \min(\maxlog(\bar{x}), 0)$.
This produces the approximation
\[
  \lceil \log_2 \ampl_1(\cos(\hat x)) \rceil 
  \le \maxlog \bar{x} - \minlog \bar{z} + \min(\maxlog(\bar{x}), 0).
\]

\paragraph{Tangent}
The amplification factor for $\tan(\hat{x})$
  is $|x / \tan(x) \cos^2(x^*)|$.
To bound its logarithm,
  we bound $\cos(x)$ in terms of $\tan(x)$.
Since $\sin(x)^2 + \cos(x)^2 = 1$,
  $\sqrt{1/2} \le \max(|\sin(x)|, |\cos(x)|) \le 1$.
Divide both sides by $|\cos(x)|$
  and take the logarithm;
  this yields:
\[
  -\frac12 - \log_2 |\cos(x)| \le \max(\log_2 |\tan(x)|, 0) \le
  - \log_2 |\cos(x)|,
\]
  or, in other words,
\[
  - 2 \log_2 |\cos(x)| \in
  2\max(\log_2(|\tan(x)|), 0) + [0, 1],
\]
  leaving
\begin{align*}
\lceil \log_2\ampl_1(\tan(\hat{x})) \rceil
&\le
\maxlog \bar{x} - \minlog \bar{z} + 2 \max(\maxlog \bar{z}, 0) + 1 \\
&= \maxlog \bar{x} - \minlog \bar{z} + \maxlog \bar{z} + \max(\maxlog \bar{z}, -\maxlog \bar{z}) + 1 \\
&= \maxlog \bar{x} + |\maxlog \bar{z}| + \logspan \bar{z} + 1,
\end{align*}
  which now only uses already-computed intervals
  and is at most one bit from being tight.

\paragraph{Arctangent}
The amplification factor for the arctangent
  contains a $x / (x^2 + 1)$ term,
  which we must bound in terms of $x$.
Some rearrangement yields
\[
\log_2 \left| \frac{x}{x^2 + 1} \right|
= - \log_2 \left| x + \frac1x \right|.
\]
Now consider $x \ge 1$;
  for these inputs, we clearly have
\[
  \log_2 |x + 1/x| \ge \log_2 |x| = \left|\log_2 |x|\right|
\]
Since the left- and right-hand sides
  are both invariant under both
  $x \mapsto 1/x$ and $x \mapsto -x$,
  this inequality is then true for all $x$.
Moreover, this approximation is off by at most one bit.

\paragraph{Hyperbolic Functions}

The amplification factors for $\sinh$ and $\cosh$
  both use $\tanh(x)$.
Because $|\tanh(x)| \le \min(|x|, 1)$,
  we have
  $\lceil \log_2 |\tanh(x)| \rceil \le \min(\maxlog(\bar{x}), 0)$,
  the approximation being off by at most one bit.

The amplification factor for $\tanh(x)$
  requires bounding $x / \sinh(x) \cosh(x)$.
We use a very weak bound,
  $x / \sinh(x) \cosh(x) \le 1$,
  which is only tight near 0.
